When Evidence and Significance Collide

Null hypothesis statistical significance testing (NHST) is the dominant approach for evaluating results from randomized controlled trials. Whereas NHST comes with long-run error rate guarantees, its main inferential tool -- the $p$-value -- is only an indirect measure of evidence against the null hypothesis. The main reason is that the $p$-value is based on the assumption the null hypothesis is true, whereas the likelihood of the data under any alternative hypothesis is ignored. If the goal is to quantify how much evidence the data provide for or against the null hypothesis it is unavoidable that an alternative hypothesis be specified (Goodman & Royall, 1988). Paradoxes arise when researchers interpret $p$-values as evidence. For instance, results that are surprising under the null may be equally surprising under a plausible alternative hypothesis, such that a $p=.045$ result (`reject the null') does not make the null any less plausible than it was before. Hence, $p$-values have been argued to overestimate the evidence against the null hypothesis. Conversely, it can be the case that statistically non-significant results (i.e., $p>.05)$ nevertheless provide some evidence in favor of the alternative hypothesis. It is therefore crucial for researchers to know when statistical significance and evidence collide, and this requires that a direct measure of evidence is computed and presented alongside the traditional $p$-value.

==> tables/simulation_sequential_short.tex <==
\begin{sidewaystable}[ph!]
\caption{Probability (SE) of finding support for the null hypothesis ($H_0$), alternative hypothesis ($H_1$), or not reaching a decision (undecided) in the simulated sequential analysis and the mean time in months (SE) of finding support for either the null or alternative hypothesis for each simulation condition comparing Bayesian model-averaging (BMA) to model selection using information (AIC, BIC), model selection using Bayes factors (BF), excluding the parametric models corresponding to the true data generating process. Results the model selection with AIC /  BIC correspond to k = 20 steps in a sequential analysis with binding asymmetric boundaries, Hwang-Shih-DeCani spending function, and $\alpha = 0.05$ for one-sided test.}
\label{tab:simulation_sequential_short}

\footnotesize
\begin{tabular}{l|rrr|rrr}
    \multicolumn{1}{l}{\multirow{2}{*}{\textbf{Decision}}} & \multicolumn{3}{c}{log(AF) = -.20} & \multicolumn{3}{|c}{log(AF) = 0} \\
    & \multicolumn{1}{|c}{$H_0$} & \multicolumn{1}{c}{Undecided} & \multicolumn{1}{c|}{$H_1$} & \multicolumn{1}{|c}{$H_0$} & \multicolumn{1}{c}{Undecided} & \multicolumn{1}{c}{$H_1$} \\
    \hline
    BMA  & 0.998 (0.002) & 0.000 (0.000) & 0.002 (0.002) & 0.896 (0.014) & 0.048 (0.010) & 0.056 (0.010) \\ 
    BF   & 0.998 (0.002) & 0.000 (0.000) & 0.002 (0.002) & 0.884 (0.014) & 0.056 (0.010) & 0.060 (0.011) \\ 
    AIC  & 1.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.930 (0.011) & 0.042 (0.009) & 0.028 (0.007) \\ 
    BIC  & 1.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.930 (0.011) & 0.042 (0.009) & 0.028 (0.007)  \\ 
    \hline
    \\
    
    \multicolumn{1}{l}{\multirow{2}{*}{\textbf{Decision}}} & \multicolumn{3}{c}{log(AF) = 0.20} & \multicolumn{3}{|c}{log(AF) = 0.40} \\
    & \multicolumn{1}{|c}{$H_0$} & \multicolumn{1}{c}{Undecided} & \multicolumn{1}{c|}{$H_1$} & \multicolumn{1}{|c}{$H_0$} & \multicolumn{1}{c}{Undecided} & \multicolumn{1}{c}{$H_1$} \\
    \hline
    BMA  & 0.184 (0.017) & 0.136 (0.015) & 0.680 (0.021) & 0.016 (0.006) & 0.008 (0.004) & 0.976 (0.007) \\ 
    BF   & 0.164 (0.017) & 0.152 (0.016) & 0.684 (0.021) & 0.016 (0.006) & 0.008 (0.004) & 0.976 (0.007) \\ 
    AIC  & 0.112 (0.014) & 0.212 (0.018) & 0.676 (0.021) & 0.006 (0.003) & 0.012 (0.005) & 0.982 (0.006) \\ 
    BIC  & 0.116 (0.014) & 0.208 (0.018) & 0.676 (0.021) & 0.006 (0.003) & 0.012 (0.005) & 0.982 (0.006) \\ 

    \hline
\end{tabular}
\\
\\

\begin{tabular}{l|rr|rr||rrr}
    \multicolumn{1}{l}{\multirow{2}{*}{\textbf{Time}}} & \multicolumn{2}{c}{log(AF) = -0.20} & \multicolumn{2}{|c||}{log(AF) = 0} & \multicolumn{3}{c}{Average} \\
    & \multicolumn{1}{|c}{$H_0$} & \multicolumn{1}{c|}{$H_1$} & \multicolumn{1}{|c}{$H_0$} & \multicolumn{1}{c||}{$H_0$} & 
    \multicolumn{1}{|c}{$H_0$} & \multicolumn{1}{c}{$H_1$} & \multicolumn{1}{c}{$H_0$ or $H_1$} \\
    \hline
    BMA  & 5.3 (0.14) & 4.0.0 (--) & 10.6 (0.36) & 7.0 (0.96) & 7.8 (0.21) & 6.9 (0.93) & 7.8 (0.20) \\ 
    BF   & 5.6 (0.15) & 4.0.0 (--) & 11.4 (0.41) & 8.1 (0.97) & 8.3 (0.23) & 7.9 (0.95) & 8.3 (0.22) \\ 
    AIC  & 8.5 (0.18) & 0.0 (--) & 19.6 (0.52) & 29.3 (4.60) & 13.9 (0.32) & 29.3 (4.60) & 14.1 (0.33) \\ 
    BIC  & 8.4 (0.18) & 0.0 (--) & 19.6 (0.52) & 29.0 (4.57) & 13.8 (0.32) & 29.0 (4.57) & 14.0 (0.33) \\ 
    \hline
    \\
    
    \multicolumn{1}{l}{\multirow{2}{*}{\textbf{Time}}} & \multicolumn{2}{c}{log(AF) = 0.20} & \multicolumn{2}{|c||}{log(AF) = 0.40} & \multicolumn{3}{c}{Average} \\
    & \multicolumn{1}{|c}{$H_0$} & \multicolumn{1}{c|}{$H_1$} & \multicolumn{1}{|c}{$H_0$} & \multicolumn{1}{c||}{$H_0$} & 
    \multicolumn{1}{|c}{$H_0$} & \multicolumn{1}{c}{$H_1$} & \multicolumn{1}{c}{$H_0$ or $H_1$} \\
    \hline
    BMA  & 11.1 (0.76) & 14.0 (0.55) & 7.8 (1.31) & 8.7 (0.27) & 10.8 (0.71) & 10.8 (0.29) & 10.8 (0.27) \\ 
    BF   & 11.6 (0.89) & 13.9 (0.54) & 8.8 (1.31) & 8.7 (0.26) & 11.4 (0.82) & 10.8 (0.28) & 10.9 (0.27) \\ 
    AIC  & 29.7 (2.15) & 28.5 (0.71) & 12.5 (5.07) & 16.9 (0.32) & 28.8 (2.11) & 21.6 (0.40) & 22.1 (0.40) \\  
    BIC  & 28.9 (2.08) & 28.3 (0.72) & 11.9 (5.57) & 16.6 (0.33) & 28.1 (2.05) & 21.4 (0.40) & 21.9 (0.41) \\ 
    \hline
\end{tabular}

\end{sidewaystable}
